Gated Delta Networks: Improving Mamba2 with Delta Rule

Linear Transformers have gained attention as efficient alternatives to standard Transformers, but their performance in retrieval and long-context tasks has been limited. To address these limitations, recent work has explored two distinct mechanisms: gating for adaptive memory control and the delta update rule for precise memory modifications. We observe that these mechanisms are complementary: gating enables rapid memory erasure while the delta rule facilitates targeted updates. Building on this insight, we introduce the gated delta rule and develop a parallel training algorithm optimized for modern hardware. Our proposed architecture, Gated DeltaNet, consistently surpasses existing models like Mamba2 and DeltaNet across multiple benchmarks, including language modeling, common-sense reasoning, in-context retrieval, length extrapolation, and long-context understanding. We further enhance performance by developing hybrid architectures that combine Gated DeltaNet layers with sliding window attention or Mamba2 layers, achieving both improved training efficiency and superior task performance.

==> figures/length.tex <==
\begin{figure}
\centering
\begin{tikzpicture}
    \begin{axis}[
            width=11cm,
            height=6cm,
            % grid=both,
            ymajorgrids=true,
            xmajorgrids=true,
            tickwidth=0pt,
            tick align=inside,
            axis line style={opacity=0},
            % minor grid style={gray!25},
            % major grid style={gray!25},
            % xlabel={Input Length},
            xtick={2000, 8000, 14000, 20000, 26000, 32000},
            ytick={13, 14, 15, 16},
            xticklabels={2K, 8K, 14K, 20K, 26K, 32K},
            scaled ticks=false,
            ylabel={\footnotesize PPL ($\downarrow$)},
            xlabel={Position bucket},
            ylabel style={font=\footnotesize,at={(0.05,0.5)}},
            ymax=16.5,
            ymin=12.5,
            legend entries={DeltaNet, Mamba2, Gated DeltaNet},
            % legend pos=south east,
            legend style={
                    font=\footnotesize,
                    legend columns=4,
                    at={(0.5,1.)},
                    anchor=north,
                },
            % restrict y to domain=8.6:10,
            % clip=true,
        ]

        % \begin{scope}[on above layer]
        %     \node[anchor=south east, rounded corners=5pt, anchor=west, align=center, draw=gray] (commit) at ($(axis cs: 2048, 10) + (10pt, 0pt)$) {\textcolor{red}{TODO: Something like}\\ Xfmr's PPL blow up!};
        %     \draw[-, thin, shorten <=0pt, shorten >=2.8pt, out=180, in=0, gray] (commit) to ($(axis cs: 2048, 10) + (0pt, 2pt)$);
        % \end{scope}

        \addplot[
            densely dashdotted,
            mark=square*, draw=red!50, thick,
            mark size=0.8pt,
            mark options={fill=red!50, fill opacity=1.0, solid},
            opacity=1.0,
        ] coordinates {
                ( 2048, 16.44)
                ( 4096, 13.73)
                ( 6144, 13.71)
                ( 8192, 13.75)
                (10240, 13.86)
                (12288, 13.97)
                (14336, 14.14)
                (16384, 14.30)
                (18432, 14.44)
                (20480, 14.63)
                (22528, 14.85)
                (24576, 15.05)
                (26624, 15.32)
                (28672, 15.60)
                (30720, 15.90)
                (32000, 16.15)
            };

        \addplot[
            dotted,
            mark=x, draw=blue!70, thick,
            mark size=2pt,
            mark options={
                    % fill=white,
                    fill opacity=0.5,
                    solid},
            opacity=1.0,
        ] coordinates {
                ( 2048, 15.58)
                ( 4096, 13.30)
                ( 6144, 13.31)
                ( 8192, 13.40)
                (10240, 13.56)
                (12288, 13.69)
                (14336, 13.83)
                (16384, 13.89)
                (18432, 13.91)
                (20480, 13.94)
                (22528, 13.96)
                (24576, 13.94)
                (26624, 13.94)
                (28672, 13.94)
                (30720, 13.95)
                (32000, 13.96)
            };

        \addplot[
            densely dashed,
            mark=pentagon*, draw=orange!70, thick,
            mark size=1.2pt,
            mark options={
                    fill=orange!70,
                    fill opacity=1.0, solid
                },
            opacity=1.0,
        ] coordinates {
                ( 2048, 15.45)
                ( 4096, 13.09)
                ( 6144, 13.12)
                ( 8192, 13.14)
                (10240, 13.17)
                (12288, 13.19)
                (14336, 13.23)
                (16384, 13.24)
                (18432, 13.22)
                (20480, 13.22)
                (22528, 13.22)
                (24576, 13.18)
                (26624, 13.18)
                (28672, 13.17)
                (30720, 13.17)
                (32000, 13.17)
            };

        \draw [semithick, black] (axis description cs:0,0) -- (axis description cs:1,0); % This line adds a thick line at y=0
        \draw [semithick, black] (axis description cs:0,1) -- (axis description cs:1,1); % This line adds a thick line at y=1
    \end{axis}


\end{tikzpicture}
\caption{Length extrapolation results in PG19 test set~\citep{pg19}. We split , and only evaluate perplexity within that bucket. }
\label{figure:}
\end{figure}
